A Deep Learning Approach To Multiple Kernel Fusion

Kernel fusion is a popular and effective approach for combining multiple features that characterize different aspects of data. Traditional approaches for Multiple Kernel Learning (MKL) attempt to learn the parameters for combining the kernels through sophisticated optimization procedures. In this paper, we propose an alternative approach that creates dense embeddings for data using the kernel similarities and adopts a deep neural network architecture for fusing the embeddings. In order to improve the effectiveness of this network, we introduce the kernel dropout regularization strategy coupled with the use of an expanded set of composition kernels. Experiment results on a real-world activity recognition dataset show that the proposed architecture is effective in fusing kernels and achieves state-of-the-art performance.

==> conclusion.tex <==
In this paper we present a deep learning approach to multiple kernel fusion by exploiting the similarity measures in kernels as feature and transform the kernel fusion problems into a feature learning problem. The framework is general and more advanced techniques can be easily incorporated into the stages such as dense embedding and fusion layer. Future plans include evaluating the architecture on more datasets and extend it to applications that contain temporal information.  
